KV Cache Compression, But What Must We Give in Return? A Comprehensive Benchmark of Long Context Capable Approaches

Long context capability is a crucial competency for large language models (LLMs) as it mitigates the human struggle to digest long-form texts. This capability enables complex task-solving scenarios such as book summarization, code assistance, and many more tasks that are traditionally manpower-intensive. However, transformer-based LLMs face significant challenges with long context input due to the growing size of the KV cache and the intrinsic complexity of attending to extended inputs; where multiple schools of efficiency-driven approaches - such as KV cache quantization, token dropping, prompt compression, linear-time sequence models, and hybrid architectures - have been proposed to produce efficient yet long context-capable models. Despite these advancements, no existing work has comprehensively benchmarked these methods in a reasonably aligned environment. In this work, we fill this gap by providing a taxonomy of current methods and evaluating 10+ state-of-the-art approaches across seven categories of long context tasks. Our work reveals numerous previously unknown phenomena and offers insights - as well as a friendly workbench - for the future development of long context-capable LLMs. The source code is available at https://github.com/henryzhongsc/longctx_bench.

==> figures/needle_latex/needle_latex_template.tex <==
% four needles in a row, single column
% four needles in a row, single column
% three needles in a row, single column.
% six needles in two row, single column is also acceptable. kivi-only

\begin{figure*}[h]
\setlength{\abovecaptionskip}{0mm}
\setlength{\belowcaptionskip}{-6mm}
\centering
\subfigcapskip=-2mm
\subfigure[]{
\centering
	\begin{minipage}[t]{0.23\linewidth}
		\includegraphics[width=\linewidth]{figures/needle/needle_template_nopad.pdf}
	\end{minipage}%
}
\subfigure[]{
\centering
	\begin{minipage}[t]{0.23\linewidth}
		\includegraphics[width=\linewidth]{figures/needle/needle_template_nopad.pdf}
	\end{minipage}%
}
\subfigure[]{
\centering
	\begin{minipage}[t]{0.23\linewidth}
		\includegraphics[width=\linewidth]{figures/needle/needle_template_nopad.pdf}
	\end{minipage}%
}
\subfigure[]{
\centering
	\begin{minipage}[t]{0.23\linewidth}
		\includegraphics[width=\linewidth]{figures/needle/needle_template_nopad.pdf}
	\end{minipage}%
}
\caption{demo: 4 needle charts without bar no padding}
\label{fig:needle_wo_bar}
\end{figure*}


==> tables/main_table_mistral.tex <==

\begin{table*}[ht]
\centering
\caption{Performance of KV cache quantization, token eviction, and prompt compression methods on Mistral-7B in our benchmark.}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|l|c|cccccc|cc}
\toprule
Model      & Method & Comp. Ratio & Single. QA & Multi. QA & Summ. & Few-shot & Synthetic & Code & LB Avg & Needle \\
\midrule
\multirow{20}{*}{\rotatebox[origin=c]{90}{Mistral-7B-Instruct-v0.2}} & Baseline & 1.00$\times$ & 32.5 & 25.8 & 27.9 & 66.8 & 89.3 & 52.4 & 43.5 & 100.0 \\
        & \rowcolor{LightCyan} KIVI-2bit & 5.05$\times$ & 31.4 & 24.7 & 27.6 & 66.8 & 80.8 & 52.1 & 42.4 & 99.0 \\
        & KIVI-4bit & 3.11$\times$ & 32.3 & 25.8 & 28.0 & 66.9 & 89.4 & 52.4 & 43.5 & 99.0 \\
        & \rowcolor{LightCyan} FlexGen-4bit & 3.20$\times$ & 31.7 & 25.1 & 27.6 & 65.9 & 82.3 & 52.4 & 42.5 & 98.3 \\
        & InfLLM-2x & 2.00$\times$ & 30.7 & 24.7 & 26.7 & 65.1 & 65.8 & 51.5 & 40.7 & 64.3 \\
        & \rowcolor{LightCyan} InfLLM-4x & 4.00$\times$ & 25.5 & 23.8 & 25.6 & 63.2 & 42.4 & 51.5 & 37.3 & 31.6 \\
        & InfLLM-6x & 6.00$\times$ & 23.9 & 21.0 & 24.9 & 61.4 & 32.4 & 50.7 & 35.2 & 32.0 \\
        & \rowcolor{LightCyan} InfLLM-8x & 8.00$\times$ & 22.6 & 20.3 & 24.4 & 61.2 & 23.9 & 50.3 & 34.0 & 28.3 \\
        & StreamLLM-2x & 2.00$\times$ & 24.3 & 22.1 & 25.3 & 64.6 & 47.1 & 50.9 & 37.2 & 54.7 \\
        & \rowcolor{LightCyan} StreamLLM-4x & 4.00$\times$ & 20.4 & 19.9 & 23.3 & 61.2 & 31.6 & 50.8 & 33.8 & 32.0 \\
        & StreamLLM-6x & 6.00$\times$ & 18.4 & 16.0 & 22.1 & 59.7 & 25.3 & 52.1 & 31.9 & 25.0 \\
        & \rowcolor{LightCyan} StreamLLM-8x & 8.00$\times$ & 17.3 & 15.2 & 21.4 & 58.7 & 16.9 & 52.5 & 30.6 & 19.3 \\
        & $\mathrm{H_2O}$-2x & 2.00$\times$ & 35.7 & 29.7 & 26.7 & 66.8 & 84.8 & 53.8 & 44.6 & 97.3 \\
        & \rowcolor{LightCyan} $\mathrm{H_2O}$-4x & 4.00$\times$ & 34.3 & 28.7 & 24.9 & 67.2 & 83.5 & 53.1 & 43.7 & 93.3 \\
        & $\mathrm{H_2O}$-6x & 6.00$\times$ & 33.7 & 28.2 & 24.3 & 66.9 & 82.7 & 52.5 & 43.2 & 86.0 \\
        & \rowcolor{LightCyan} $\mathrm{H_2O}$-8x & 8.00$\times$ & 32.8 & 27.6 & 23.6 & 67.0 & 84.2 & 52.3 & 42.8 & 79.7 \\
        & LLMLingua2-2x & 2.00$\times$ & 28.4 & 23.0 & 26.5 & 45.3 & 54.9 & 30.9 & 32.4 & 42.0 \\
        & \rowcolor{LightCyan} LLMLingua2-4x & 4.00$\times$ & 25.1 & 21.3 & 24.6 & 39.0 & 14.0 & 32.0 & 27.2 & 10.7 \\
        & LLMLingua2-6x & 6.00$\times$ & 21.2 & 17.4 & 23.3 & 38.6 & 8.9 & 33.3 & 25.1 & 0.3 \\
        & \rowcolor{LightCyan} LLMLingua2-8x & 8.00$\times$ & 19.6 & 16.1 & 22.9 & 38.0 & 8.0 & 34.0 & 24.4 & 0.0 \\
\bottomrule
\end{tabular}
}
\label{tab:main_table_mistral}
\end{table*}
